Quantitative results on the Ishikawa iteration of Lipschitz pseudo-contractions

We compute uniform rates of metastability for the Ishikawa iteration of a Lipschitz pseudo-contractive self-mapping of a compact convex subset of a Hilbert space. This extraction is an instance of the proof mining program that aims to apply tools from mathematical logic in order to extract the hidden quantitative content of mathematical proofs. We prove our main result by applying methods developed by Kohlenbach, the first author and Nicolae for obtaining quantitative versions of strong convergence results for generalized Fej\'er monotone sequences in compact subsets of metric spaces.

==> macros.tex <==

\usepackage{a4wide}
\usepackage{amscd}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{array}
\usepackage{color}
%\usepackage{diagrams}
\usepackage{epsfig}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage[colorlinks=true,urlcolor=blue,linkcolor=blue,plainpages=false,pdfpagelabels
]{hyperref}
\usepackage{ifthen}
\usepackage{tabularx}
\usepackage{url}
\usepackage[all,cmtip]{xy}


%\usepackage{MnSymbol} 

%%%%%%%%%%PENTRU CURS: SEMINARII SI TEME


\newcommand{\veranstaltung}{Ergodic Theory and Additive Combinatorics}
\newcommand{\veranstalter}{Lauren\c tiu Leu\c stean}
\newcommand{\semester}{Summer Term 2013}
\newcommand{\nummer}{1}
\newcommand{\datum}{01.10.2010}
\newcommand{\beschreibung}{Seminar \blattno}

\newcounter{uebno}
%\newcommand{\datum}{26.10.2010}
%\newcommand{\beschreibung}{Seminar \blattno}


\newsavebox{\uebung}
%\savebox{\uebung}{\raisebox{-11pt}{\parbox[t]{6cm}{\bf SNSB\\ \noindent \semester\\ \veranstaltung\\
%                                          \veranstalter}}}

\newcommand{\titel}{ 
\usebox{\uebung}  
\bigskip
\begin{flushright} \datum \end{flushright}
\vspace{2mm}
\begin{center}{\Large \bf 
\beschreibung }
 \end{center} \vspace{5mm}
}

\newcommand{\homex}{\stepcounter{uebno}{\vspace{0.3cm}\noindent \bf (H\blattno.\arabic{uebno}) }}
\newcommand{\semex}{\stepcounter{uebno}{\vspace{0.3cm}\noindent \bf (S\blattno.\arabic{uebno}) }}
\newcommand{\probex}{\stepcounter{uebno}{\vspace{0.3cm}\noindent \bf (P\blattno.\arabic{uebno}) }}

%%%%%%%%%%%%%%%%%%%
\newenvironment{denseBibitem}[1]
{\bibitem{#1}\begin{minipage}[t]{\textwidth}}
{\end{minipage}}

\providecommand{\defnterm}[1]{\textbf{#1}}

\newcommand{\solution}[1]{\begin{proof}#1\end{proof}}
\newcommand{\easyfacts}[1]{{\bf EASY-begin} #1 {\bf EASY-end}\\}
\newcommand{\solapp}[1]{\begin{proof}#1\end{proof}}
\newcommand{\solsem}[1]{\begin{proof}#1\end{proof}}
\newcommand{\soleasy}[1]{\begin{proof} {\bf EASY SOLUTION} #1\end{proof}}
\newcommand{\solex}[1]{\begin{proof}#1\end{proof}}
\newcommand{\solhom}[1]{\begin{proof}#1\end{proof}}
\newcommand{\soltowritebetter}[1]{\begin{proof} {\bf  TO WRITE BETTER} #1\end{proof}}
\newcommand{\comment}[1]{***COMMENT {\,\,\bf #1}***}
\newcommand{\details}[1]{$\,$\\***DETAILS {\bf #1}***\\}
\newcommand{\solutionsem}[1]{} %%% are solutia in seminar. Dar o scriu totusi si in lecture notes.



\newtheorem{theorem}{Theorem}[section]
%\makeatletter
%\@addtoreset{theorem}{chapter}
%\@addtoreset{theorem}{section}
%\@addtoreset{theorem}{appendix}
%\makeatother

\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Remark}
\newtheorem{exemplu}[theorem]{Example}
\newtheorem{exercise}{Exercise}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{problem}[theorem]{Problem}

\newcommand{\bdfn}{\begin{definition}}
\newcommand{\edfn}{\end{definition}}
\newcommand{\bthm}{\begin{theorem}}
\newcommand{\ethm}{\end{theorem}}
\newcommand{\bprop}{\begin{proposition}}
\newcommand{\eprop}{\end{proposition}}
\newcommand{\bcor}{\begin{corollary}}
\newcommand{\ecor}{\end{corollary}}
\newcommand{\blem}{\begin{lemma}}
\newcommand{\elem}{\end{lemma}}
\newcommand{\bfact}{\begin{fact}}
\newcommand{\efact}{\end{fact}}
\newcommand{\bex}{\begin{exemplu}\begin{rm}}
\newcommand{\eex}{\end{rm}\end{exemplu}}
\newcommand{\bxc}{\begin{exercise}}
\newcommand{\exc}{\end{exercise}}
\newcommand{\bntn}{\begin{notation}}
\newcommand{\entn}{\end{notation}}

\newcommand{\note}{\medskip \noindent {\bf Not\v{a}:} \hspace{1ex}}
\newcommand{\foo}[1]{\footnote{#1}}
\newcommand{\bb}[1]{\bbold {#1}}

\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bce}{\begin{center}}
\newcommand{\ece}{\end{center}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bt}{\begin{tabular}}
\newcommand{\et}{\end{tabular}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ba}{\begin{array}} 
\newcommand{\ea}{\end{array}}
\newcommand {\bea} {\begin{eqnarray}}
\newcommand {\eea} {\end {eqnarray}}
\newcommand {\bua} {\begin{eqnarray*}}
\newcommand {\eua} {\end {eqnarray*}}

\newcommand{\defi}{:\,\,=}

\newcommand{\bm}{\boldmath}
\newcommand{\sra}{\rightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\hra}{\hookrightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\Ba}{\Leftrightarrow}
\newcommand{\se}{\subseteq}
\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}
\newcommand{\dis}{\displaystyle}
\newcommand{\lan}{\left\langle}
\newcommand{\ran}{\right\rangle}
\newcommand{\ua}{\!\!\uparrow\!\!}
\newcommand{\da}{\!\!\downarrow\!\!}
\newcommand{\ca}{\leadsto}
\newcommand{\Lra}{\Leftrightarrow}

\newcommand{\vsp}{\vspace*}
\newcommand{\hsp}{\hspace*}

\newcommand{\uae}{The following are equivalent}
\newcommand{\notatie}{\stackrel{\rm not}{=}}
\newcommand{\ds}{\displaystyle}



\providecommand{\defnterm}[1]{\textbf{#1}}

\newcounter{ct}
\newenvironment{ilist}{\begin{list}{\rm (\roman{ct})}{\usecounter{ct}\labelwidth1.2cm\leftmargin1cm
\itemsep0ex\topsep.4ex}}{\end{list}}
%
\newenvironment{alist}{\begin{list}{(\arabic{ct})}{\usecounter{ct}\labelwidth1cm\leftmargin1.5cm
}}{\end{list}}

\renewcommand{\labelenumi}{(\roman{enumi})}
\renewcommand{\labelenumii}{(\alph{enumii})}
\renewcommand{\labelenumiii}{(\arabic{enumiii})}
\renewcommand{\labelenumiv}{(\Alph{enumiv})}

\renewcommand{\theenumi}{\roman{enumi}}

%%% MATE GENERAL %%%


\newcommand{\nelem}{\in\!\!\!\!/\,}
\newcommand{\ninclus}{\subseteq\!\!\!\!\!/\,}

%Parantheses

\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left[}
\newcommand{\rb}{\right]}


\def\R{{\mathbb R}}
\def\N{{\mathbb N}}
\def\Z{{\mathbb Z}}
\def\C{{\mathbb C}}
\def\K{{\mathbb K}}
\def\Q{{\mathbb Q}}
\def\B{{\mathbb B}}
\def\E{{\mathbb E}}
\def\R{{\mathbb R}}
\def\S{{\mathbb S}}
\def\T{{\mathbb T}}
\def\H{{\mathbb H}}
\newcommand\M{{\mathbf{M}}}
\newcommand\I{{\mathcal{I}}}
\newcommand\X{{\mathcal{X}}}
\newcommand\Y{{\mathcal{Y}}}

\newcommand{\Nat}{{\mathbb N}}
\newcommand{\Real}{{\mathbb R}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}

\newcommand{\av}{\mathbf{a}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\zv}{\mathbf{z}}
\newcommand{\uv}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\nv}{\mathbf{n}}


\newcommand{\vp}{\varphi}
\newcommand{\eps}{\varepsilon}


\newcommand{\remin}{\mathop{-\!\!\!\!\!\hspace*{1mm}\raisebox{0.5mm}{$
\cdot$}}\nolimits}

\newcommand{\limn}{\ds\lim_{n\to\infty}}
\newcommand{\limk}{\ds\lim_{k\to\infty}}
\newcommand{\limh}{\ds\lim_{h\to\infty}}
\newcommand{\limm}{\ds\lim_{m\to\infty}}
\newcommand{\limN}{\ds\lim_{N\to\infty}}
\newcommand{\lsupn}{\ds \limsup_{n\to\infty}}
\newcommand{\linfn}{\ds\liminf_{n\to\infty}}
\newcommand{\linfN}{\ds\liminf_{N\to\infty}}



\newcommand{\infn}{\ds\inf_{n\to\infty}}
\newcommand{\supn}{\ds\sup_{n\to\infty}}

\newcommand{\plim}{p\!-\!\lim}
\newcommand{\plimxn}{\plim x_n}
\newcommand{\plimcxn}{\plim cx_n}
\newcommand{\plimfxn}{\plim f(x_n)}
\newcommand{\plimyn}{\plim y_n}
\newcommand{\plimxyn}{\plim (x_n+y_n)}





%%% GEODESIC %%%%

\newcommand{\lambdaxy}{(1-\lambda)x\oplus\lambda y}
\newcommand{\tlambdaxy}{(1-\tilde{\lambda})x\oplus\tilde{\lambda} y}
\newcommand{\midxy}{\frac12x\oplus\frac12y}
\newcommand{\midyz}{\frac12y\oplus\frac12z}
\newcommand{\tlambda}{\tilde{\lambda}}
\newcommand{\xylambda}{xy_\lambda}
\newcommand{\geoxy}{Geod_{xy}}
\newcommand{\geoxx}{Geod_{xx}}
\newcommand{\geosegxy}{GeodSeg_{xy}}
\newcommand{\geosegxx}{GeodSeg_{xy}}
\newcommand{\geowxy}{W_{xy}}
\newcommand{\geowpxy}{W'_{xy}}
\newcommand{\geowcxy}{W_{xy}^*}
\newcommand{\geowpcxy}{W'_{xy}^*}

%%% LOGICA %%% 

\newcommand{\aquant}{\forall}
\newcommand{\equant}{\exists}
\newcommand{\si}{\wedge}
\newcommand{\sau}{\vee}
\newcommand{\dnd}{\leftrightarrow}
\newcommand{\smaj}{\,s\! -\! maj}
\newcommand{\ssmaj}{\,ss\! -\! maj}
\newcommand{\amaj}{{\mathop{>}_{\sim}}^a}
\newcommand{\bmaj}{{\mathop{>}_{\sim}}^b}
\newcommand{\amajrho}{{\mathop{>}_{\sim}}^a_\rho}

\newcommand{\adw}{{\cal A}^\omega[X,d,W]_{-b}}


\newcommand{\aomega}{{\cal A}^\omega}
\newcommand{\aomegaxd}{\mathcal{A}^\omega[X,d]_{-b}}
\newcommand{\aomegaxdw}{\mathcal{A}^\omega[X,d,W]_{-b}}
\newcommand{\aomegaxducw}{\mathcal{A}^\omega[X,d,UCW,\eta]_{-b}}
\newcommand{\aomegan}{\mathcal{A}^\omega[X,\|\cdot\|]}
\newcommand{\epaomega}{E\!-\!PA^\omega}
\newcommand{\wehaomega}{WE\!-\!HA^\omega}


%%%measure theory 

\providecommand{\defnterm}[1]{\textbf{#1}}
\newcommand{\sigalg}{$\sigma$-algebra }
\newcommand{\sigring}{$\sigma$-ring }
\newcommand{\sigfin}{$\sigma$-finite}
\long\def\daggerfn#1{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[2]{#1}\endgroup}


\newcommand{\seqAn}{\lbrace A_n\rbrace}
\newcommand{\mus}{\mu^*}
\newcommand{\mmus}{\cM(\mu^*)}
\newcommand{\sigs}{\sigma(\cS)}


\newcommand{\cupinA}{\bigcup_{i=1}^nA_i}
\newcommand{\suminA}{\sum_{i=1}^n\mu(A_i)}
\newcommand{\cupinC}{\bigcup_{i=1}^nC_i}


\newcommand{\cupnA}{\bigcup_{n=1}^\infty A_n}
\newcommand{\sumnA}{\sum_{n=1}^\infty\mu(A_n)}
\newcommand{\cupincF}{\bigcup_{i=1}^\cF_i}
\newcommand{\cupncF}{\bigcup_{n=1}^\infty \cF_n}



\newcommand{\muss}{\mus_{\sigma(\cS)}}
\newcommand{\musm}{\mus_{\cM(\mus)}}


\newcommand{\extR}{\tilde{\R}}
\newcommand{\extRk}{\tilde{\R}^k}
\newcommand{\extB}{\tilde{\cB}}
\newcommand{\extBk}{\tilde{\cB^k}}
\newcommand{\infv}{\mathbf{+\infty}}
\newcommand{\infmv}{\mathbf{-\infty}}


\newcommand{\Agen}{\cA}
\newcommand{\Rgen}{\cR}

\newcommand{\amc}{at most countable}
\newcommand{\card}[1]{|#1|}
\newcommand{\cardR}{\text{card}(\cR)}

%%measurable spaces, mappings

\newcommand{\measpX}{(X,\cB)}
\newcommand{\measpXC}{(X,\cC)}
\newcommand{\measpY}{(Y,\cC)}
\newcommand{\measpZ}{(Z,\cD)}

\newcommand{\meatraR}{\cM_\R(X,\cB)}
\newcommand{\meatraC}{\cM_\C(X,\cB)}
\newcommand{\meatraRX}{\cM_\R(X,\cB)}
\newcommand{\meatraCX}{\cM_\C(X,\cB)}
\newcommand{\meatraRY}{\cM_\R(Y,\cC)}
\newcommand{\meatraCY}{\cM_\C(Y,\cC)}
\newcommand{\meatraRZ}{\cM_\R(Z,\cD)}
\newcommand{\meatraCZ}{\cM_\C(Z,\cD)}


%%measure spaces


\newcommand{\msp}{(X,\cB,\mu)}
\newcommand{\mspX}{(X,\cB,\mu)}
\newcommand{\mspY}{(Y,\cC,\nu)}
\newcommand{\mspXC}{(X,\cC,\mu)}
\newcommand{\mspZ}{(Z,\cD,\psi)}


\newcommand{\cmspY}{(\ol{Y},\ol{\cC},\ol{\nu})}
\newcommand{\cmspX}{(\ol{X},\ol{\cB},\ol{\mu})}


%%probability spaces

\newcommand{\probsp}{(X,\cB,\mu)}
\newcommand{\probspX}{(X,\cB,\mu)}
\newcommand{\probspY}{(Y,\cC,\nu)}
\newcommand{\probspZ}{(Z,\cD,\eta)}


%%measure-preserving systemns

\newcommand{\mpsXT}{(X,\cB,\mu,T)}
\newcommand{\mpsYS}{YX,\cC,\nu,S)}


\newcommand{\mpt}{measure-preserving transformation}
\newcommand{\mps}{measure-preserving system}
\newcommand{\imps}{invertible measure-preserving system}
\newcommand{\pmps}{probability measure-preserving system}
\newcommand{\sigmainvT}{\cB^T}


%% Lp spaces

\newcommand{\LpX}{L^p\mspX}
\newcommand{\LpY}{L^p\mspY}
\newcommand{\LpRX}{L^p_\R\mspX}
\newcommand{\LpRY}{L^p_\R\mspY}
\newcommand{\LdX}{L^2\mspX}
\newcommand{\LuX}{L^1\mspX}
\newcommand{\LuRX}{L^1_\R\mspX}
\newcommand{\LuXC}{L^1\mspXC}
\newcommand{\LuRXC}{L^1_\R\mspXC}
\newcommand{\LdXC}{L^2\mspXC}
\newcommand{\LdRX}{L^2_\R\mspX}
\newcommand{\LpXC}{L^p\mspXC}
\newcommand{\LpRXC}{L^p_\R\mspXC}

\def\esssup{\text{ess sup}}
\newcommand{\LiX}{L^\infty\mspX}
\newcommand{\LiY}{L^\infty\mspY}
\newcommand{\LiRX}{L^\infty_\R\mspX}
\newcommand{\LiRY}{L^\infty_\R\mspY}

\newcommand{\mpXY}{{\cM\cP}_{XY}}
\newcommand{\impXY}{{\cI\cM\cP}_{XY}}

\newcommand{\tma}{T^{-1}(A)}
\newcommand{\tmb}{T^{-1}(B)}
\newcommand{\tmdna}{T^{-2n}(A)}
\newcommand{\tmna}{T^{-n}(A)}
\newcommand{\tmia}{T^{-i}(A)}
\newcommand{\tmka}{T^{-k}(A)}
\newcommand{\tmina}{T^{-in}(A)}
\newcommand{\tmkna}{T^{-kn}(A)}
\newcommand{\tmkmuna}{T^{-(k-1)n}(A)}
\newcommand{\tmNa}{T^{-N}(A)}
\newcommand{\tmc}{T^{-1}(C)}
\newcommand{\tmnc}{T^{-n}(C)}
\newcommand{\tmkc}{T^{-k}(C)}
\newcommand{\tmNc}{T^{-N}(C)}



\newcommand{\muae}{$\mu$-aFe. } 
\newcommand{\intef}{\int_E f}
\newcommand{\tie}{\tilde{\cI}_E}
\newcommand{\tief}{\tilde{\cI}_E(f)}
\newcommand{\tieg}{\tilde{\cI}_E(g)}
\newcommand{\tiff}{\tilde{\cI}_F(f)}
\newcommand{\tifg}{\tilde{\cI}_F(g)}
\newcommand{\lue}{L^1(E)}
\newcommand{\luaee}{L^1_{ae}(E)}


\newcommand{\sumfTx}{\frac1n\sum_{k=0}^{n-1}f(T^kx)}
\newcommand{\sumfUx}{\frac1n\sum_{k=0}^{n-1}f(U^kx)}
\newcommand{\sumfU}{\frac1n\sum_{k=0}^{n-1}f\circ U^k}

\newcommand{\snfTx}{\sum_{k=0}^{n-1}f(T^kx)}
\newcommand{\prodfTx}{\prod_{k=0}^{n-1}f(T^kx)}

\newcommand{\mutmnab}{\mu(\tmna\cap B)}
\newcommand{\mutmiab}{\mu(\tmia\cap B)}
\newcommand{\Snmix}{\frac1n\sum_{i=0}^{n-1}\mutmiab}
\newcommand{\Snxn}{\frac1n\sum_{i=0}^{n-1}x_i}
\newcommand{\Snxnm}{\frac1n\sum_{i=0}^{n-1<}x_i|}
\newcommand{\Snxnd}{\frac1n\sum_{i=0}^{n-1}x_i^2}

\newcommand{\DlimnE}{\lim_{n\to\infty\atop{n\notin E}}}
\newcommand{\DlimhE}{\lim_{h\to\infty\atop{h\notin E}}}
\newcommand{\Dlimh}{D\!-\!\lim_{h\to\infty}}
\newcommand{\Dlimn}{D\!-\!\lim_{n\to\infty}}

\newcommand{\cexpC}{E(\cdot|\cC)}
\newcommand{\cexpfC}{E(f|\cC)}
\newcommand{\cexpgC}{E(g|\cC)}


%%%%%%%%%%%%%%%RAMSEY THEORY%%%%%%%%%%%%%%%%%%%

\newcommand{\fsxn}{FS\big((x_n)_{n\ge 1}\big)}
\newcommand{\fsxun}{FS\big((x_k)_{k=1}^n\big)}
\newcommand{\fsxunu}{FS\big((x_k)_{k=1}^{n+1}\big)}
\newcommand{\fsnl}{FS\big(n_1,\ldots, n_l\big)}
\newcommand{\fpar}{\bigcup_{i=1}^r C_i}


%%%%%%%%%%%%%%%Density%%%%%%%%%%%%%%%%%%%

\newcommand{\uBd}{Bd^\star}
\newcommand{\lBd}{Bd_\star}
\newcommand{\Bd}{Bd}

\newcommand{\ud}{\ol{d}}
\newcommand{\ld}{\ul{d}}


%%%%%%%%%%%%%%%Ergodic Theory%%%%%%%%%%%%%%%%%%%

\newcommand{\snf}{S_nf}
\newcommand{\eavf}{A_nf}
\newcommand{\eavuf}{A_{n+1}f}
\newcommand{\eavmf}{A_n(-f)}
\newcommand{\eavmodf}{A_n(|f|)}
\newcommand{\eavfA}{A_n\chi_A}
\newcommand{\eavfB}{A_n\chi_B}

%%% SPACES %%%%

\newcommand{\torusn}{\cT^n}
\newcommand{\torus}{\cT}
\newcommand{\sphere}{\cS^1}
\newcommand{\nsphere}{\cS^n}

%%% FUNCTIONAL ANALYSIS

\newcommand{\xnwx}{x_n\stackrel{w}{\to}x}
\newcommand{\Txnwx}{Tx_n\stackrel{w}{\to}x}


%% TOPOLOGICAL DYNAMICAL SYSTEMS 

\newcommand{\forbx}{{\cal O}_+(x)}
\newcommand{\forbxo}{{\cal O}_+(x_0)}
\newcommand{\forby}{{\cal O}_+(y)}
\newcommand{\forbg}{{\cal O}_+(g)}
\newcommand{\forbunu}{{\cal O}_+(1)}
\newcommand{\porbx}{{\cal O}_{>0}(x)}
\newcommand{\cforbx}{\ol{\cal O}_+(x)}
\newcommand{\cforby}{\ol{\cal O}_+(y)}
\newcommand{\fuorbx}{{\cal O}_{>0}(x)}
\newcommand{\cfuorbx}{\ol{\cal O}_{>0}(x)}
\newcommand{\orbx}{{\cal O}(x)}
\newcommand{\orbg}{{\cal O}(g)}
\newcommand{\orbunu}{{\cal O}(1)}
\newcommand{\corbx}{\ol{\cal O}(x)}
\newcommand{\corbxy}{\ol{\cal O}(x,y)}

\newcommand{\stinv}{strongly $T$-invariant}
\newcommand{\tinv}{$T$-invariant }

\newcommand{{\Fdo}}{F}

%%%ULRICH

%%changed from Ulrich's one
\newcommand{\res}{\!\!\!\upharpoonright}











